Coplanar circumbinary planets can be unstable to large tilt oscillations in the presence of an inner polar planet

Mutually misaligned circumbinary planets may form in a warped or broken gas disc or from later planet-planet interactions. With numerical simulations and analytic estimates we explore the dynamics of two circumbinary planets with a large mutual inclination. A coplanar inner planet causes prograde apsidal precession of the binary and the stationary inclination for the outer planet is higher for larger outer planet orbital radius. In this case a coplanar outer planet always remains coplanar. On the other hand, a polar inner planet causes retrograde apsidal precession of the binary orbit and the stationary inclination is smaller for larger outer planet orbital radius. For a range of outer planet semi-major axes, an initially coplanar orbit is librating meaning that the outer planet undergoes large tilt oscillations. Circumbinary planets that are highly inclined to the binary are difficult to detect -- it is unlikely for a planet to have an inclination below the transit detection limit in the presence of a polar inner planet. These results suggest that there could be a population of circumbinary planets that are undergoing large tilt oscillations.

==> RESPONSE.tex <==
We thank the referee very much for the timely report and the useful comments that have improved the manuscript. We strongly feel that our findings are well suited for publication in ApJL.  The main finding in this letter, that an initially coplanar circumbinary planet can undergo large tilt oscillations in the presence of a highly inclined inner planet, is surprising and holds significant implications for current and future observations.  This newly identified dynamical behavior may help to explain current circumbinary planet demographics.  Furthermore, we believe we have sufficiently addressed all of the suggested changes within the limits of a letter.  We respectfully request that this manuscript be considered as a letter for publication in ApJL.

Reviewer's Comments:

The authors studied the dynamics of two planets in a circumbinary system, where the inner planet is highly inclined (in a polar orbit) with respect to the stellar binary, and the outer planet is coplanar with the stellar binary. The authors find that the outer planet can have large inclination variations even if it starts coplanar with respect to the stellar binary. The results are interesting and the writing is very clear. However, I find the analysis to be quite crude (e.g., the authors neglected the nodal precession of the outer planet due to the inner planet, and it is not clear what exactly caused the flip). Thus, I'd like to recommend some revisions. 

In addition, I think the paper would be better suited to the main ApJ, instead of ApJ Letters, since it seems rather unsurprising that the coplanar outer planet can have large inclination variations due to the inclined inner planet and then be flipped. In addition, this may allow a more extensive analysis of the dynamics.

Major comments: 

1. The analysis in section 3 seems very crude. It seems the authors neglected the nodal precession of the outer planet due to the inner giant planet (based on eqn 3-7). There's no discussion of why the effect of the inner planet on the outer planet is neglected. The precession rate of the outer planet due to the inner planet can be larger than \dot{\varpi_b} depending on the location of the planets, so it may be important to include this term. 

RESPONSE: We have numerically evolved the evolution of the outer particle ignoring the forcing from the inner planet and we find very little difference in the dynamics of the outer planet, highlighting that the dynamics are indeed driven by the binary precession and not the planet--planet interactions.  We have added a discussion of this to Section 3. 

In addition, the analytical results are not well compared with numerical results, so it is not clear how robust/accurate are the analytical estimates. Specifically, the authors only compared the calculated critical radii in Figs 2 and 3, but Fig 2 only included a few examples with large gaps in a_p2. For instance, it may be nice to add a plot of the maximum inclination of the initially coplanar outer planet as a function of a_p2 to compare with r_c1, r_c2 and r_c3 more quantitatively, and to also test the results for different a_p1 values.

RESPONSE:   We have compared numerical results to our analytic predictions for r_c1 and r_c2 by adding our numerical values to Figure 4.  We have removed our analytic predictions for r_c3 as we choose to focus on the surprising behavior of a librating planet in the presence of an inner polar planet.  To probe the effect of a_p2, Figure 3 shows the maximum inclination of the outer initially coplanar planet as a function of a_p2. The top left panel of figure 4 considers different a_p1 values.


2. The numerical results illustrate clearly the flip of the outer planet. However, the analysis (section 3) doesn't show clearly how exactly the orbit is flipped, i.e., what caused the bifurcation as the inner planet inclination increases as shown in the numerical results. Is it driven by the precession of the binary due to the inner planet or the perturbation of the outer planet by the inner planet? Is it possible to provide a better understanding (or an analytical estimate) of the critical inclination of the inner planet that leads to the flip of the outer planet? It seems a lot more analysis can be done to improve our understanding of the dynamics.

RESPONSE:  In the last paragraph of Section 3 we have added a calculation of the ratio of the nodal precession of the outer planet driven by the inner planet and also the ratio of the nodal precession of the outer planet driven by the binary.  We further demonstrate that the dynamics of the outer planet are indeed driven by the precession rate of the binary.  


Minor comments:

1. In the analysis, the authors adopted the nodal phase angle (\phi), instead of the more conventional "longitude of ascending node" to study the nodal precession. It is not clear why the authors made this choice. The nodal phase angle is measured relative to the binary orbit, which is changing. On the other hand, the conventional longitude of ascending node is measured relative to a fixed reference plane and conjugate to the z-component of angular momentum. It may be more straight forward to analyze the dynamics using the standard canonical variables (e.g., to interpret the results using the constant energy contours to study the libration and circulation regions).

RESPONSE:  We choose to use the nodal phase angle in the frame of the binary for consistency with previous literature.  Farago \& Laskar, Chen et al., and Childs \& Martin, among others, use this notation. The phase diagrams in figure 2 would be messy if we did not work in the frame of the binary.

2. In the introduction, the authors motivated this study referring to the warping of the circumbinary disk. However, it seems the outer planet needs to be very close to the binary (~20ab) in order to have large inclination variations. It will be nice to include some discussions on the possibilities of the warping close to the binaries.

RESPONSE: The radius at which the disc breaks depends on the disc aspect ratio and viscosity and properties of the binary, but for standard parameters the disc can break close to the binary, well within 10ab (see Nixon2013, Facchini2013, and Lubow2018).  Furthermore, other mechanisms that may result in CBP misalignment include multiple accretion events onto a binary that can form misaligned discs (Bate2018).  We have added discussion of this to the introduction.

3. In the numerical example in section 2, it will be better to use a case of unequal mass binary. The unequal mass binaries are quite common, and the unequal mass binaries will lead to non-zero octupole effects (e.g., Naoz et al. 2016 eqn 5) and be more general, unless the author would like to choose a more specific (simpler) case for illustration.

RESPONSE: We have recreated the phase diagrams of Figure 2 using q=0.5 and find little difference to the equal mass binary presented.  This is in agreement with Chen et al 2019 who found that the binary fraction had little effect on the dynamics of two circumbinary planets with small mutual inclinations (see Figure 1, models A1 and B1 of Chen 2019), only the timescale.  In Figure 4 we may see that the critical radii are relatively insensitive to the binary mass fraction. Furthermore, the eccentricity of both circumbinary planets is ~0 meaning the octupole term goes to zero.  We have added this point to Section 2.

4. For Figure 5, it may not be necessary to distinguish those starting less or higher than 90 deg, since the over dynamics can be well illustrated in the i\cos(phi) and i\sin(phi) plane already. The different colors may make the plots too busy.

RESPONSE:  In regards to Figure 2, we chose the color scheme, and to distinguish between orbits less than and greater than 90 degree, for consistency with previous literature and we prefer to keep it this way.  Please see Chen et al. 2019, Doolin et al. 2011.

5. The discussion in line 215-218 seems not well supported. It sounds very strange that the dynamics of the outer planet is dominated more by the binary than the inner planet when the outer planet moves closer to the inner planet. It may be helpful to calculate the precession rates due to binary and the inner planet separately to clarify this.

RESPONSE: We have evolved the system (binary+inner polar planet+outer test particle) and removed the planet-planet interaction. We find a difference in the tilt evolution of just a few percent. So the precession of the outer planet due to the inner planet is negligible.  We have added a discussion of this in Section 3.

6. It would be nice to provide more quantitative comparisons between numerical N-body simulations and the analytical results on the three critical semi-major axes.

RESPONSE:  We have marked our numerical results on Figure 4 and find good agreement for r_c1 and r_c2 with our analytical predictions.

7. It may be nice also to compare the critical radii with disk warping radii to illustrate how applicable are the dynamical results to circumbinary systems (e.g., around line 305-307).

RESPONSE: We estimate the disk breaking radius using equation (34) of Lubow2018.  Assuming the fiducial disk parameters of Lubow2018, a disk aspect ratio of H/R=0.05, and our binary parameters, the disk breaking radius is approximately 2.8 a_b.  This is in agreement with simulations of similar disks and permits for an inner highly misaligned planet and an outer planet beyond r_c1.  We have added these points to Section 3.

==> Two body circumbinary planet dynamics with large mutual inclinations/RESPONSE.tex <==
We thank the referee very much for the timely report and the useful comments that have improved the manuscript. We strongly feel that our findings are well suited for publication in ApJL.  The main finding in this letter, that an initially coplanar circumbinary planet can undergo large tilt oscillations in the presence of a highly inclined inner planet, is surprising and holds significant implications for current and future observations.  This newly identified dynamical behavior may help to explain current circumbinary planet demographics.  Furthermore, we believe we have sufficiently addressed all of the suggested changes within the limits of a letter.  We respectfully request that this manuscript be considered as a letter for publication in ApJL.

Reviewer's Comments:

The authors studied the dynamics of two planets in a circumbinary system, where the inner planet is highly inclined (in a polar orbit) with respect to the stellar binary, and the outer planet is coplanar with the stellar binary. The authors find that the outer planet can have large inclination variations even if it starts coplanar with respect to the stellar binary. The results are interesting and the writing is very clear. However, I find the analysis to be quite crude (e.g., the authors neglected the nodal precession of the outer planet due to the inner planet, and it is not clear what exactly caused the flip). Thus, I'd like to recommend some revisions. 

In addition, I think the paper would be better suited to the main ApJ, instead of ApJ Letters, since it seems rather unsurprising that the coplanar outer planet can have large inclination variations due to the inclined inner planet and then be flipped. In addition, this may allow a more extensive analysis of the dynamics.

Major comments: 

1. The analysis in section 3 seems very crude. It seems the authors neglected the nodal precession of the outer planet due to the inner giant planet (based on eqn 3-7). There's no discussion of why the effect of the inner planet on the outer planet is neglected. The precession rate of the outer planet due to the inner planet can be larger than \dot{\varpi_b} depending on the location of the planets, so it may be important to include this term. 

RESPONSE: We have numerically evolved the evolution of the outer particle ignoring the forcing from the inner planet and we find very little difference in the dynamics of the outer planet, highlighting that the dynamics are indeed driven by the binary precession and not the planet--planet interactions.  We have added a discussion of this to Section 3. 

In addition, the analytical results are not well compared with numerical results, so it is not clear how robust/accurate are the analytical estimates. Specifically, the authors only compared the calculated critical radii in Figs 2 and 3, but Fig 2 only included a few examples with large gaps in a_p2. For instance, it may be nice to add a plot of the maximum inclination of the initially coplanar outer planet as a function of a_p2 to compare with r_c1, r_c2 and r_c3 more quantitatively, and to also test the results for different a_p1 values.

RESPONSE:   We have compared numerical results to our analytic predictions for r_c1 and r_c2 by adding our numerical values to Figure 4.  We have removed our analytic predictions for r_c3 as we choose to focus on the surprising behavior of a librating planet in the presence of an inner polar planet.  To probe the effect of a_p2, Figure 3 shows the maximum inclination of the outer initially coplanar planet as a function of a_p2. The top left panel of figure 4 considers different a_p1 values.


2. The numerical results illustrate clearly the flip of the outer planet. However, the analysis (section 3) doesn't show clearly how exactly the orbit is flipped, i.e., what caused the bifurcation as the inner planet inclination increases as shown in the numerical results. Is it driven by the precession of the binary due to the inner planet or the perturbation of the outer planet by the inner planet? Is it possible to provide a better understanding (or an analytical estimate) of the critical inclination of the inner planet that leads to the flip of the outer planet? It seems a lot more analysis can be done to improve our understanding of the dynamics.

RESPONSE:  In the last paragraph of Section 3 we have added a calculation of the ratio of the nodal precession of the outer planet driven by the inner planet and also the ratio of the nodal precession of the outer planet driven by the binary.  We further demonstrate that the dynamics of the outer planet are indeed driven by the precession rate of the binary.  


Minor comments:

1. In the analysis, the authors adopted the nodal phase angle (\phi), instead of the more conventional "longitude of ascending node" to study the nodal precession. It is not clear why the authors made this choice. The nodal phase angle is measured relative to the binary orbit, which is changing. On the other hand, the conventional longitude of ascending node is measured relative to a fixed reference plane and conjugate to the z-component of angular momentum. It may be more straight forward to analyze the dynamics using the standard canonical variables (e.g., to interpret the results using the constant energy contours to study the libration and circulation regions).

RESPONSE:  We choose to use the nodal phase angle in the frame of the binary for consistency with previous literature.  Farago \& Laskar, Chen et al., and Childs \& Martin, among others, use this notation. The phase diagrams in figure 2 would be messy if we did not work in the frame of the binary.

2. In the introduction, the authors motivated this study referring to the warping of the circumbinary disk. However, it seems the outer planet needs to be very close to the binary (~20ab) in order to have large inclination variations. It will be nice to include some discussions on the possibilities of the warping close to the binaries.

RESPONSE: The radius at which the disc breaks depends on the disc aspect ratio and viscosity and properties of the binary, but for standard parameters the disc can break close to the binary, well within 10ab (see Nixon2013, Facchini2013, and Lubow2018).  Furthermore, other mechanisms that may result in CBP misalignment include multiple accretion events onto a binary that can form misaligned discs (Bate2018).  We have added discussion of this to the introduction.

3. In the numerical example in section 2, it will be better to use a case of unequal mass binary. The unequal mass binaries are quite common, and the unequal mass binaries will lead to non-zero octupole effects (e.g., Naoz et al. 2016 eqn 5) and be more general, unless the author would like to choose a more specific (simpler) case for illustration.

RESPONSE: We have recreated the phase diagrams of Figure 2 using q=0.5 and find little difference to the equal mass binary presented.  This is in agreement with Chen et al 2019 who found that the binary fraction had little effect on the dynamics of two circumbinary planets with small mutual inclinations (see Figure 1, models A1 and B1 of Chen 2019), only the timescale.  In Figure 4 we may see that the critical radii are relatively insensitive to the binary mass fraction. Furthermore, the eccentricity of both circumbinary planets is ~0 meaning the octupole term goes to zero.  We have added this point to Section 2.

4. For Figure 5, it may not be necessary to distinguish those starting less or higher than 90 deg, since the over dynamics can be well illustrated in the i\cos(phi) and i\sin(phi) plane already. The different colors may make the plots too busy.

RESPONSE:  In regards to Figure 2, we chose the color scheme, and to distinguish between orbits less than and greater than 90 degree, for consistency with previous literature and we prefer to keep it this way.  Please see Chen et al. 2019, Doolin et al. 2011.

5. The discussion in line 215-218 seems not well supported. It sounds very strange that the dynamics of the outer planet is dominated more by the binary than the inner planet when the outer planet moves closer to the inner planet. It may be helpful to calculate the precession rates due to binary and the inner planet separately to clarify this.

RESPONSE: We have evolved the system (binary+inner polar planet+outer test particle) and removed the planet-planet interaction. We find a difference in the tilt evolution of just a few percent. So the precession of the outer planet due to the inner planet is negligible.  We have added a discussion of this in Section 3.

6. It would be nice to provide more quantitative comparisons between numerical N-body simulations and the analytical results on the three critical semi-major axes.

RESPONSE:  We have marked our numerical results on Figure 4 and find good agreement for r_c1 and r_c2 with our analytical predictions.

7. It may be nice also to compare the critical radii with disk warping radii to illustrate how applicable are the dynamical results to circumbinary systems (e.g., around line 305-307).

RESPONSE: We estimate the disk breaking radius using equation (34) of Lubow2018.  Assuming the fiducial disk parameters of Lubow2018, a disk aspect ratio of H/R=0.05, and our binary parameters, the disk breaking radius is approximately 2.8 a_b.  This is in agreement with simulations of similar disks and permits for an inner highly misaligned planet and an outer planet beyond r_c1.  We have added these points to Section 3.
